Proceedings of the Low-$x$ 2021 International Workshop

The purpose of the Low-$x$ Workshop series is to stimulate discussions between experimentalists and theorists in diffractive hadronic physics, QCD dynamics at low $x$, parton saturation, and exciting problems in QCD at HERA, Tevatron, LHC, RHIC, and the future EIC. The central topics of the workshop, summarized in the current Proceedings, were: Diffraction in ep and e-ion collisions (including EIC physics); Diffraction and photon-exchange in hadron-hadron, hadron-nucleus, and nucleus-nucleus collisions; Spin Physics; Low-$x$ PDFs, forward physics, and hadronic final states. This Workshop has been the XXVIII edition in the series of the workshop.

==> Precision_QCD_measurements_from_CMS/Precision_QCD_measurements_from_CMS/x.tex <==
\relax 
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyperFirstAtBeginDocument{\AtBeginDocument}
\HyperFirstAtBeginDocument{\ifx\hyper@anchor\@undefined
\global\let\oldcontentsline\contentsline
\gdef\contentsline#1#2#3#4{\oldcontentsline{#1}{#2}{#3}}
\global\let\oldnewlabel\newlabel
\gdef\newlabel#1#2{\newlabelxx{#1}#2}
\gdef\newlabelxx#1#2#3#4#5#6{\oldnewlabel{#1}{{#2}{#3}}}
\AtEndDocument{\ifx\hyper@anchor\@undefined
\let\contentsline\oldcontentsline
\let\newlabel\oldnewlabel
\fi}
\fi}
\global\let\hyper@last\relax 
\gdef\HyperFirstAtBeginDocument#1{#1}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{CMS-PAS-SMP-18-014}
\citation{CMS-PAS-SMP-21-006}
\citation{CMS-PAS-SMP-21-009}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-JINST-3-S08004}
\citation{CMS-PAS-SMP-20-011}
\babel@aux{english}{}
\@writefile{toc}{\contentsline {section}{\numberline {1}Introduction}{1}{section.1}}
\citation{CMS-PAS-SMP-18-014}
\citation{CMS-PAS-SMP-18-014}
\@writefile{toc}{\contentsline {section}{\numberline {2}Precision measurement of the Z invisible width at $\sqrt  {s} = 13\ensuremath  {\tmspace  +\thinmuskip {.1667em}\text  {Te\hspace  {-.08em}V}\xspace  }$}{2}{section.2}}
\newlabel{ZinvisibleWidth}{{2.1}{2}{Precision measurement of the Z invisible width at $\sqrt {s} = 13\TeV $}{equation.2.1}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces Missing transverse momentum $\ensuremath  {p_\mathrm  {T}}^{\mathrm  {miss}}$ distributions. Selected charged leptons do not contribute to $\ensuremath  {p_\mathrm  {T}}^{\mathrm  {miss}}$. Also shown are the ratios with respect to the SM postfit and the residuals as the difference between data and SM postfit.~\cite  {CMS-PAS-SMP-18-014}\relax }}{2}{figure.caption.1}}
\providecommand*\caption@xref[2]{\@setref\relax\@undefined{#1}}
\newlabel{ZinvisibleWidthData}{{1}{2}{Missing transverse momentum $\pt ^{\mathrm {miss}}$ distributions. Selected charged leptons do not contribute to $\pt ^{\mathrm {miss}}$. Also shown are the ratios with respect to the SM postfit and the residuals as the difference between data and SM postfit.~\cite {CMS-PAS-SMP-18-014}\relax }{figure.caption.1}{}}
\citation{CMS-PAS-SMP-18-014}
\citation{CMS-PAS-SMP-18-014}
\citation{CMS-PAS-SMP-21-009}
\citation{Nagy:2001fj}
\citation{Britzger:2012bs}
\citation{Currie:2016bfm}
\citation{Dulat:2015mca}
\citation{CMS-PAS-SMP-21-009}
\citation{CMS-PAS-SMP-21-009}
\citation{CMS-PAS-SMP-21-009}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces Comparison of the $\ensuremath  {\mathrm  {Z}}$ invisible width measurement with the direct measurements from the experiments at the LEP. The present measurement is in good agreement with the LEP combination~\cite  {CMS-PAS-SMP-18-014}.\relax }}{3}{figure.caption.2}}
\newlabel{ZinvisibleWidth}{{2}{3}{Comparison of the $\PZ $ invisible width measurement with the direct measurements from the experiments at the LEP. The present measurement is in good agreement with the LEP combination~\cite {CMS-PAS-SMP-18-014}.\relax }{figure.caption.2}{}}
\@writefile{toc}{\contentsline {section}{\numberline {3}Measurement of the double-differential inclusive jet cross section at 5\ensuremath  {\tmspace  +\thinmuskip {.1667em}\text  {Te\hspace  {-.08em}V}\xspace  }}{3}{section.3}}
\citation{Alwall:2014hca}
\citation{Baranov:2021uol}
\citation{Sjostrand:2014zea}
\citation{CMS:2015wcf}
\citation{CMS:2015wcf}
\citation{BermudezMartinez:2018fsv}
\citation{Alwall:2014hca}
\citation{BermudezMartinez:2018fsv}
\citation{CMS-PAS-SMP-21-006}
\citation{CMS-PAS-SMP-21-006}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces A comparison of the 5\ensuremath  {\tmspace  +\thinmuskip {.1667em}\text  {Te\hspace  {-.08em}V}\xspace  }inclusive jet cross section data to theory predictions at NLO using the $H_T$ scale (left), at NLO using the $\ensuremath  {p_\mathrm  {T}}$ scale (middle) and at NNLO using the $H_T$ scale~\cite  {CMS-PAS-SMP-21-009}.\relax }}{4}{figure.caption.3}}
\newlabel{5TeVdataVsTheory}{{3}{4}{A comparison of the 5\TeV inclusive jet cross section data to theory predictions at NLO using the $H_T$ scale (left), at NLO using the $\pt $ scale (middle) and at NNLO using the $H_T$ scale~\cite {CMS-PAS-SMP-21-009}.\relax }{figure.caption.3}{}}
\@writefile{toc}{\contentsline {section}{\numberline {4}Cross section measurements of jet multiplicity and jet transverse momenta in multijet events at 13\ensuremath  {\tmspace  +\thinmuskip {.1667em}\text  {Te\hspace  {-.08em}V}\xspace  }}{4}{section.4}}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-PAS-SMP-20-011}
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces A comparison of the measured $\ensuremath  {p_\mathrm  {T}}$ distributions of the 3rd and 4th leading jets to NLO predictions~\cite  {CMS-PAS-SMP-21-006}.\relax }}{5}{figure.caption.4}}
\newlabel{multijetFig}{{4}{5}{A comparison of the measured $\pt $ distributions of the 3rd and 4th leading jets to NLO predictions~\cite {CMS-PAS-SMP-21-006}.\relax }{figure.caption.4}{}}
\@writefile{toc}{\contentsline {section}{\numberline {5}Measurement and QCD analysis of double-differential inclusive jet cross sections at 13\ensuremath  {\tmspace  +\thinmuskip {.1667em}\text  {Te\hspace  {-.08em}V}\xspace  }}{5}{section.5}}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-PAS-SMP-20-011}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces \textit  {Left:} The inclusive jet cross sections with a comparison to NLO QCD predictions using the CT14 PDF~\cite  {CMS-PAS-SMP-20-011}. \textit  {Right:} The probability matrix. The horizontal and vertical axes correspond to particle and detector level jets, respectively.~\cite  {CMS-PAS-SMP-20-011}\relax }}{6}{figure.caption.5}}
\newlabel{13TeV_cs_and_rm}{{5}{6}{\textit {Left:} The inclusive jet cross sections with a comparison to NLO QCD predictions using the CT14 PDF~\cite {CMS-PAS-SMP-20-011}. \textit {Right:} The probability matrix. The horizontal and vertical axes correspond to particle and detector level jets, respectively.~\cite {CMS-PAS-SMP-20-011}\relax }{figure.caption.5}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces Comparisons of the double differential cross section data to theoretical predictions using different PDFs and portraying the role of various uncertainties. In the bottom plot all histograms are divided by the NLO+NLL prediction and in the top plot by the NNLO prediction, obtained using the CT14 PDF~\cite  {CMS-PAS-SMP-20-011}.\relax }}{7}{figure.caption.6}}
\newlabel{13TeV_data_vs_theory}{{6}{7}{Comparisons of the double differential cross section data to theoretical predictions using different PDFs and portraying the role of various uncertainties. In the bottom plot all histograms are divided by the NLO+NLL prediction and in the top plot by the NNLO prediction, obtained using the CT14 PDF~\cite {CMS-PAS-SMP-20-011}.\relax }{figure.caption.6}{}}
\newlabel{SMfactorisation}{{5.1}{7}{Measurement and QCD analysis of double-differential inclusive jet cross sections at 13\TeV }{equation.5.1}{}}
\newlabel{SMEFT_Lagrangian}{{5.2}{7}{Measurement and QCD analysis of double-differential inclusive jet cross sections at 13\TeV }{equation.5.2}{}}
\citation{CMS-PAS-SMP-20-011}
\citation{Sirunyan:2019zvx}
\citation{Abramowicz:2015mha}
\citation{Bertone:2017tig}
\citation{Gao:2012qpa}
\citation{Paukkunen:2014zia}
\citation{Dulat:2015mca}
\citation{Sirunyan:2019zvx}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-PAS-SMP-20-011}
\citation{Abramowicz:2015mha}
\citation{Sirunyan:2019zvx}
\citation{10.1093/ptep/ptaa104}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces Results of profiling with the CT14nlo PDF at NLO. The utilized CMS data are the inclusive jet and the triple-differential \ensuremath  {{\ensuremath  {\mathrm  {t}}{}\overline  {\ensuremath  {\mathrm  {t}}}}}cross sections at $\sqrt  {s}=13\ensuremath  {\tmspace  +\thinmuskip {.1667em}\text  {Te\hspace  {-.08em}V}\xspace  }$. \textit  {Left:} Relative uncertainty in the gluon distribution, shown as a function of the momentum fraction $x$ for the scale $\mu _\text  {f}=m_\ensuremath  {\mathrm  {t}}$. The original CT14 uncertainty is shown in red and the profiling result in blue~\cite  {CMS-PAS-SMP-20-011}. \textit  {Right:} The $\chi ^2$ scan obtained in profiling $\ensuremath  {\alpha _S}(m_\ensuremath  {\mathrm  {Z}})$ using the CT14 PDF series~\cite  {CMS-PAS-SMP-20-011}.\relax }}{8}{figure.caption.8}}
\newlabel{profilingPlots}{{7}{8}{Results of profiling with the CT14nlo PDF at NLO. The utilized CMS data are the inclusive jet and the triple-differential \ttbar cross sections at $\sqrt {s}=13\TeV $. \textit {Left:} Relative uncertainty in the gluon distribution, shown as a function of the momentum fraction $x$ for the scale $\mu _\text {f}=m_\PQt $. The original CT14 uncertainty is shown in red and the profiling result in blue~\cite {CMS-PAS-SMP-20-011}. \textit {Right:} The $\chi ^2$ scan obtained in profiling $\alpS (m_\PZ )$ using the CT14 PDF series~\cite {CMS-PAS-SMP-20-011}.\relax }{figure.caption.8}{}}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-PAS-SMP-20-011}
\citation{ZEUS:2019cou}
\citation{ATLAS:2017eqx}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces The $\ensuremath  {\mathrm  {u}}$ valence~(upper left), $\ensuremath  {\mathrm  {d}}$ valence~(upper right), gluon~(lower left), and sea quark~(lower right) PDFs as functions of the momentum fraction $x$ at the scale $\mu _\text  {f}=m_\ensuremath  {\mathrm  {t}}^2$. The red hashed band results from the SMEFT fit with the left-handed CI model using $\Lambda =10\ensuremath  {\tmspace  +\thinmuskip {.1667em}\text  {Te\hspace  {-.08em}V}\xspace  }$. It is in good agreement with the gray band resulting from the SM fit, with all differences well within the fit uncertainties~\cite  {CMS-PAS-SMP-20-011}.\relax }}{9}{figure.caption.9}}
\newlabel{SM_vs_CI_PDFs}{{8}{9}{The $\PQu $ valence~(upper left), $\PQd $ valence~(upper right), gluon~(lower left), and sea quark~(lower right) PDFs as functions of the momentum fraction $x$ at the scale $\mu _\text {f}=m_\PQt ^2$. The red hashed band results from the SMEFT fit with the left-handed CI model using $\Lambda =10\TeV $. It is in good agreement with the gray band resulting from the SM fit, with all differences well within the fit uncertainties~\cite {CMS-PAS-SMP-20-011}.\relax }{figure.caption.9}{}}
\citation{CMS-PAS-SMP-20-011}
\citation{CMS-PAS-SMP-20-011}
\bibcite{CMS-PAS-SMP-18-014}{{1}{}{{}}{{}}}
\bibcite{CMS-PAS-SMP-21-006}{{2}{}{{}}{{}}}
\bibcite{CMS-PAS-SMP-21-009}{{3}{}{{}}{{}}}
\bibcite{CMS-PAS-SMP-20-011}{{4}{}{{}}{{}}}
\bibcite{CMS-JINST-3-S08004}{{5}{}{{}}{{}}}
\bibcite{Sirunyan:2019zvx}{{6}{}{{}}{{}}}
\bibcite{Abramowicz:2015mha}{{7}{}{{}}{{}}}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces The Wilson coefficients $c_1$ obtained in the NLO SMEFT analysis, divided by $\Lambda ^2$. The black error bars show the fit uncertainty at 68\% CL. The red (blue) lines correspond to the total uncertainty at 68\% (95\%) CL~\cite  {CMS-PAS-SMP-20-011}.\relax }}{10}{figure.caption.10}}
\newlabel{13TeV_data_vs_theory}{{9}{10}{The Wilson coefficients $c_1$ obtained in the NLO SMEFT analysis, divided by $\Lambda ^2$. The black error bars show the fit uncertainty at 68\% CL. The red (blue) lines correspond to the total uncertainty at 68\% (95\%) CL~\cite {CMS-PAS-SMP-20-011}.\relax }{figure.caption.10}{}}
\@writefile{toc}{\contentsline {section}{\numberline {6}Summary}{10}{section.6}}
\bibcite{Paukkunen:2014zia}{{8}{}{{}}{{}}}
\bibcite{Bertone:2017tig}{{9}{}{{}}{{}}}
\bibcite{Gao:2012qpa}{{10}{}{{}}{{}}}
\bibcite{Currie:2016bfm}{{11}{}{{}}{{}}}
\bibcite{Alwall:2014hca}{{12}{}{{}}{{}}}
\bibcite{BermudezMartinez:2018fsv}{{13}{}{{}}{{}}}
\citation{Baranov:2021uol}
\bibcite{ZEUS:2019cou}{{14}{}{{}}{{}}}
\bibcite{Dulat:2015mca}{{15}{}{{}}{{}}}
\bibcite{10.1093/ptep/ptaa104}{{16}{}{{}}{{}}}
\bibcite{ATLAS:2017eqx}{{17}{}{{}}{{}}}
\bibcite{Nagy:2001fj}{{18}{}{{}}{{}}}
\bibcite{Britzger:2012bs}{{19}{}{{}}{{}}}
\bibcite{Sjostrand:2014zea}{{20}{}{{}}{{}}}
\bibcite{CMS:2015wcf}{{21}{}{{}}{{}}}
\providecommand\NAT@force@numbers{}\NAT@force@numbers


==> Zhang_ATLAS/definecolor.tex <==
\input{definecolor.tex}
\definecolor{tab0}{HTML}{1f77b4}
\definecolor{tab1}{HTML}{ff7f0e}
\definecolor{tab2}{HTML}{2ca02c}
\definecolor{tab3}{HTML}{d62728}
\definecolor{tab4}{HTML}{9467bd}
\definecolor{tab5}{HTML}{8c564b}
\definecolor{tab6}{HTML}{e377c2}
\definecolor{tab7}{HTML}{7f7f7f}
\definecolor{tab8}{HTML}{bcbd22}
\definecolor{tab9}{HTML}{17becf}
\definecolor{c02}{HTML}{729fcf}
\definecolor{c01}{HTML}{3465a4}
\definecolor{c0}{HTML}{204a87}
\definecolor{c12}{HTML}{fcaf3e}
\definecolor{c11}{HTML}{f57900}
\definecolor{c1}{HTML}{ce5c00}
\definecolor{c22}{HTML}{8ae234}
\definecolor{c21}{HTML}{73d216}
\definecolor{c2}{HTML}{4e9a06}
\definecolor{c32}{HTML}{ef2929}
\definecolor{c31}{HTML}{cc0000}
\definecolor{c3}{HTML}{a40000}
\definecolor{c42}{HTML}{ad7fa8}
\definecolor{c41}{HTML}{75507b}
\definecolor{c4}{HTML}{5c3566}
\definecolor{c52}{HTML}{e9b96e}
\definecolor{c51}{HTML}{c17d11}
\definecolor{c5}{HTML}{8f5902}
\definecolor{c62}{HTML}{fce94f}
\definecolor{c61}{HTML}{edd400}
\definecolor{c6}{HTML}{c4a000}
\definecolor{tab0}{HTML}{1f77b4}
\definecolor{tab1}{HTML}{ff7f0e}
\definecolor{tab2}{HTML}{2ca02c}
\definecolor{tab3}{HTML}{d62728}
\definecolor{tab4}{HTML}{9467bd}
\definecolor{tab5}{HTML}{8c564b}
\definecolor{tab6}{HTML}{e377c2}
\definecolor{tab7}{HTML}{7f7f7f}
\definecolor{tab8}{HTML}{bcbd22}
\definecolor{tab9}{HTML}{17becf}
\definecolor{c02}{HTML}{729fcf}
\definecolor{c01}{HTML}{3465a4}
\definecolor{c0}{HTML}{204a87}
\definecolor{c12}{HTML}{fcaf3e}
\definecolor{c11}{HTML}{f57900}
\definecolor{c1}{HTML}{ce5c00}
\definecolor{c22}{HTML}{8ae234}
\definecolor{c21}{HTML}{73d216}
\definecolor{c2}{HTML}{4e9a06}
\definecolor{c32}{HTML}{ef2929}
\definecolor{c31}{HTML}{cc0000}
\definecolor{c3}{HTML}{a40000}
\definecolor{c42}{HTML}{ad7fa8}
\definecolor{c41}{HTML}{75507b}
\definecolor{c4}{HTML}{5c3566}
\definecolor{c52}{HTML}{e9b96e}
\definecolor{c51}{HTML}{c17d11}
\definecolor{c5}{HTML}{8f5902}
\definecolor{c62}{HTML}{fce94f}
\definecolor{c61}{HTML}{edd400}
\definecolor{c6}{HTML}{c4a000}


==> Zhang_ATLAS/newcommand.tex <==
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\amp}{{\CMcal
\newcommand{\as}{\alpha_{\mathrm{s}}}
\newcommand{\bs}[1]{\boldsymbol{#1}}
\newcommand{\cita}[1]{\dGreen{\it\tiny
\newcommand{\dif}{\mathrm{d}}
\newcommand{\Dt}{(\kt-z\qt)}
\newcommand{\Eth}{E_\mathrm{th}}
%\newcommand{\eff}{\mathrm{eff}}
\newcommand{\esp}[1]{{\mathrm{e}^{#1}}}
\newcommand{\GeV}{\text{
\newcommand{\imp}{\Rightarrow}
%\newcommand{\GeV}{\mathrm{GeV}}
\newcommand{\kt}{{\boldsymbol
\newcommand{\Lqcd}{\Lambda_{\mathrm
\newcommand{\lt}{{\boldsymbol
\newcommand{\MeV}{\text{
\newcommand{\Mmax}{M_{\mathrm{max}}}
\newcommand{\ord}[1]{\CMcal{O}\left(#1\right)}
\newcommand{\pol}{\epsilon}
\newcommand{\plb}[3]{{\it
\newcommand{\pt}{{\boldsymbol
\newcommand{\ps}{\!\cdot\!}
\newcommand{\qt}{{\boldsymbol
\newcommand{\tg}{\CMcal{T}}
\newcommand{\ui}{\mathrm{i}}
\newcommand{\vm}[1]{\langle
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\jets}{\textrm{jets}}
\newcommand{\kt}{\ensuremath{k_\mathrm{T}}}
\newcommand{\pt}{\ensuremath{p_\mathrm{T}}}
\newcommand{\HT}{\ensuremath{H_\mathrm{T}}}
\newcommand{\Pe}{\ensuremath{\mathrm{e}}}
\newcommand{\Pp}{\ensuremath{\mathrm{p}}}
\newcommand{\PW}{\ensuremath{\mathrm{W}}}
\newcommand{\PZ}{\ensuremath{\mathrm{Z}}}
\newcommand{\PQu}{\ensuremath{\mathrm{u}}}
\newcommand{\PQd}{\ensuremath{\mathrm{d}}}
\newcommand{\PQt}{\ensuremath{\mathrm{t}}}
\newcommand{\alpS}{\ensuremath{\alpha_S}}
\newcommand{\ttbar}{\ensuremath{{\PQt{}\overline{\PQt}}}}
\newcommand{\MeV}{\ensuremath{\,\text{Me\hspace{-.08em}V}\xspace}}
\newcommand{\GeV}{\ensuremath{\,\text{Ge\hspace{-.08em}V}\xspace}}
\newcommand{\TeV}{\ensuremath{\,\text{Te\hspace{-.08em}V}\xspace}}
\newcommand{\MADGRAPH}
\newcommand{\MGvATNLO}{\MADGRAPH{}5\_aMC@NLO\xspace}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\drv}{{\rm
\newcommand{\tild}{~}
\newcommand{\tcite}[1]{~\cite{#1}}
\newcommand{\tref}[1]{~\ref{#1}}
\newcommand{\eref}[1]{~\eqref{#1}}
\renewcommand{\arraystretch}{1.7}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand\Trule{\rule{0pt}{2.5ex}}
\newcommand\Brule{\rule[-1.ex]{0pt}{0pt}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\slv}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$v$}}
\newcommand{\sln}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$n$}}
\newcommand{\slnbar}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\bar{n}$}}
\newcommand{\slF}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$F$}}
\newcommand{\sll}{\raise.15ex\hbox{$/$}\kern-.40em\hbox{$l$}}
\newcommand{\sllbar}{\raise.15ex\hbox{$/$}\kern-.40em\hbox{$\bar{l}$}}
\newcommand{\slh}{\raise.15ex\hbox{$/$}\kern-.40em\hbox{$h$}}
\newcommand{\slP}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$P$}}
\newcommand{\slp}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$p$}}
\newcommand{\slq}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$q$}}
\newcommand{\slqbar}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\bar{q}$}}
\newcommand{\slR}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$R$}}
\newcommand{\slz}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$Z$}}
\newcommand{\slzbar}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\bar{Z}$}}
\newcommand{\slQ}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$Q$}}
\newcommand{\slK}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$K$}}
\newcommand{\slk}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$k$}}
\newcommand{\slkone}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$k_1$}}
\newcommand{\slktwo}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$k_2$}}
\newcommand{\slkthree}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$k_3$}}
\newcommand{\slkbar}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\bar{k}$}}
\newcommand{\slkbarone}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\bar{k}_1$}}
\newcommand{\slkbartwo}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\bar{k}_2$}}
\newcommand{\slkbarthree}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\bar{k}_3$}}
\newcommand{\slpone}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$p_1$}}
\newcommand{\slpbarone}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\bar{p}_1$}}
\newcommand{\slptwo}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$p_2$}}
\newcommand{\slpbartwo}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\bar{p}_2$}}
\newcommand{\slqone}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$q_1$}}
\newcommand{\slD}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\!D$}}
\newcommand{\slC}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$C$}}
\newcommand{\slA}{\raise.15ex\hbox{$/$}\kern-.73em\hbox{$A$}}
\newcommand{\slSigma}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\Sigma$}}
\newcommand{\slpartial}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\partial$}}
\newcommand{\slcalP}{\raise.15ex\hbox{$/$}\kern-.63em\hbox{$\cal
\newcommand{\sleps}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\epsilon$}}
\newcommand{\slepsbar}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\overline{\epsilon}$}}
\newcommand{\slepsstar}{\raise.15ex\hbox{$/$}\kern-.53em\hbox{$\epsilon$}^\star}
\newcommand{\slS}{\raise.15ex\hbox{$/$}\kern-.73em\hbox{$S$}}
\newcommand{\nn}{\nonumber\\}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand*{\va}{\vspace{10pt}}
\newcommand*{\vb}{\vspace{3pt}}
\newcommand*{\vm}{\vspace{-6pt}}
\newcommand{\myhref}[3][tab0]{\href{#2}{\color{#1}{#3}}}%
{\renewcommand{\arraystretch}{1.4}
{\renewcommand{\arraystretch}{1.4}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
%\newcommand{\be}{\begin{equation}}
%\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\jpsi}
\newcommand{\psip}
\newcommand{\rhozero}
\newcommand{\twohundrednn}
\newcommand{\AD}
\newcommand{\ADA}
\newcommand{\ADC}
\newcommand{\fI}
\newcommand{\fd}
%\newcommand\todo[1]{\textcolor{red}{#1}}
\newcommand{\starlight}{STARlight\xspace}
\newcommand{\montecarlo}{Monte
\newcommand{\AxE}{\ensuremath{A\times{E}}}
%
\newcommand{\pp}
\newcommand{\ppbar}
\newcommand{\XeXe}
\newcommand{\PbPb}
\newcommand{\pA}
\newcommand{\pPb}
\newcommand{\AuAu}
\newcommand{\dAu}
\newcommand{\s}
\newcommand{\snn}
\newcommand{\pt}
\newcommand{\meanpt}
\newcommand{\ycms}
\newcommand{\ylab}
\newcommand{\y}
\newcommand{\etarange}[1]
\newcommand{\yrange}[1]
\newcommand{\dndy}
\newcommand{\dndeta}
\newcommand{\avdndeta}
\newcommand{\dNdy}
\newcommand{\Npart}
\newcommand{\Ncoll}
\newcommand{\dEdx}
\newcommand{\RpPb}
\newcommand{\nineH}
\newcommand{\seven}
\newcommand{\eight}
\newcommand{\twoH}
\newcommand{\twosevensix}
\newcommand{\five}
\newcommand{\fiveExactly}
\newcommand{\twosevensixnn}{$\sqrt{s_{\mathrm{NN}}}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\fivenn}
\newcommand{\LT}
\newcommand{\GeVc}
\newcommand{\MeVc}
\newcommand{\TeV}
\newcommand{\GeV}
\newcommand{\MeV}
\newcommand{\GeVmass}
\newcommand{\MeVmass}
\newcommand{\lumi}
\newcommand{\ITS}
\newcommand{\TOF}
\newcommand{\ZDC}
\newcommand{\ZDCs}
\newcommand{\ZNA}
\newcommand{\ZNC}
\newcommand{\SPD}
\newcommand{\SDD}
\newcommand{\SSD}
\newcommand{\TPC}
\newcommand{\TRD}
\newcommand{\VZERO}
\newcommand{\VZEROA}
\newcommand{\VZEROC}
\newcommand{\Vdecay}
\newcommand{\ee}
\newcommand{\pip}
\newcommand{\pim}
\newcommand{\kap}
\newcommand{\kam}
\newcommand{\pbar}
\newcommand{\kzero}
\newcommand{\lmb}
\newcommand{\almb}
\newcommand{\Om}
\newcommand{\Mo}
\newcommand{\X}
\newcommand{\Ix}
\newcommand{\Xis}
\newcommand{\Oms}
\newcommand{\degree}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}


==> Zhang_ATLAS/newcommand_sorted.tex <==
% for paper writing in general. If other newcommands
\newcommand{\ADA}  {\rm{ADA}\xspace}
\newcommand{\ADC}  {\rm{ADC}\xspace}
\newcommand{\AD}   {\rm{AD}\xspace}
\newcommand{\almb}         {\ensuremath{\overline{\Lambda}}\xspace}
\newcommand{\amp}{{\CMcal M}}             % ampiezza
\newcommand{\as}{\alpha_{\mathrm{s}}}      % costante forte 
\newcommand{\AuAu}         {\mbox{Au--Au}\xspace}
\newcommand{\avdndeta}     {\ensuremath{\langle\dndeta\rangle}\xspace}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\be}{\begin{equation}}  
\newcommand{\cita}[1]{\dGreen{\it\tiny [#1]}}
\newcommand{\dAu}          {\mbox{d--Au}\xspace}
\newcommand{\dEdx}         {\ensuremath{\textrm{d}E/\textrm{d}x}\xspace}
\newcommand{\degree}       {\ensuremath{^{\rm o}}\xspace}
\newcommand{\dndeta}       {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}\eta}\xspace}
\newcommand{\dndy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\dNdy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\drv}{{\rm d}}
\newcommand{\eea}{\end{eqnarray}} 
%\newcommand{\eea}{\end{eqnarray}}
%\newcommand{\ee}{\end{equation}}  
\newcommand{\ee}           {\ensuremath{e^{+}e^{-}}} 
\newcommand{\eight}        {$\sqrt{s}~=~8$~Te\kern-.1emV\xspace}
\newcommand{\etarange}[1]  {\mbox{$\left | \eta \right |~<~#1$}}
\newcommand{\fd}   {f_{\rm D}}
\newcommand{\fI}   {f_{\rm I}}
\newcommand{\fiveExactly}  {$\sqrt{s}~=~5$~Te\kern-.1emV\xspace}
\newcommand{\fivenn}       {$\sqrt{s_{\mathrm{NN}}}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\five}         {$\sqrt{s}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\GeVc}         {Ge\kern-.1emV/$c$\xspace}
%\newcommand{\GeV}          {Ge\kern-.1emV\xspace}
\newcommand{\GeVmass}      {Ge\kern-.05emV/$c^2$\xspace}
\newcommand{\GeV}{\text{ GeV}}
\newcommand{\ITS}          {\rm{ITS}\xspace}
\newcommand{\Ix}           {\ensuremath{\overline{\Xi}^+}\xspace}
\newcommand{\jpsi} {\ensuremath{{\mathrm J}/\psi}\xspace}
\newcommand{\kam}          {\ensuremath{\rm{K}^{-}}\xspace}
\newcommand{\kap}          {\ensuremath{\rm{K}^{+}}\xspace}
\newcommand{\kt}{{\boldsymbol k}}
\newcommand{\kzero}        {\ensuremath{{\rm K}^{0}_{\rm{S}}}\xspace}
\newcommand{\lmb}          {\ensuremath{\Lambda}\xspace}
\newcommand{\Lqcd}{\Lambda_{\mathrm QCD}}
\newcommand{\lt}{{\boldsymbol l}}
\newcommand{\LT}           {L{\'e}vy-Tsallis\xspace}
\newcommand{\lumi}         {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\MADGRAPH} {\textsc{MadGraph}\xspace}
\newcommand{\meanpt}       {$\langle p_{\mathrm{T}}\rangle$\xspace}
\newcommand{\MeVc}         {Me\kern-.1emV/$c$\xspace}
\newcommand{\MeVmass}      {Me\kern-.05emV/$c^2$\xspace}
\newcommand{\MeV}          {Me\kern-.1emV\xspace}
%\newcommand{\MeV}{\text{ MeV}}
\newcommand{\Mo}           {\ensuremath{\overline{\Omega}^+}\xspace}
\newcommand{\montecarlo}{Monte Carlo\xspace}
\newcommand{\Ncoll}        {\ensuremath{N_\mathrm{coll}}\xspace}
\newcommand{\nineH}        {$\sqrt{s}~=~0.9$~Te\kern-.1emV\xspace}
\newcommand{\Npart}        {\ensuremath{N_\mathrm{part}}\xspace}
\newcommand{\Om}           {\ensuremath{\Omega^-}\xspace}
\newcommand{\Oms}          {\ensuremath{\Omega^{\pm}}\xspace}
\newcommand{\pA}           {\mbox{pA}\xspace}
\newcommand{\pbar}         {\ensuremath{\rm\overline{p}}\xspace}
%newcommand{\PbPb}         {\mbox{Pb--Pb}\xspace}
\newcommand{\pim}          {\ensuremath{\pi^{-}}\xspace}
\newcommand{\pip}          {\ensuremath{\pi^{+}}\xspace}
\newcommand{\plb}[3]{{\it Phys.~Lett.~}{\bf B #1} (#2) #3}
\newcommand{\ppbar}        {\mbox{$\mathrm {p\overline{p}}$}\xspace}
%\newcommand{\pPb}          {\mbox{p--Pb}\xspace}
%\newcommand{\pp}           {pp\xspace}
\newcommand{\psip} {\ensuremath{\psi'}\xspace}
%\newcommand{\pt}{{\boldsymbol p}}
\newcommand{\pt}           {\ensuremath{p_{\rm T}}\xspace}
\newcommand{\qt}{{\boldsymbol q}}
\newcommand{\rhozero} {\ensuremath{\rho^0}\xspace}
\newcommand{\RpPb}         {\ensuremath{R_{\rm pPb}}\xspace}
\newcommand{\SDD}          {\rm{SDD}\xspace}
\newcommand{\s}            {\ensuremath{\sqrt{s}}\xspace}
\newcommand{\seven}        {$\sqrt{s}~=~7$~Te\kern-.1emV\xspace}
\newcommand{\slcalP}{\raise.15ex\hbox{$/$}\kern-.63em\hbox{$\cal P$}}
\newcommand{\snn}          {\ensuremath{\sqrt{s_{\mathrm{NN}}}}\xspace}
\newcommand{\SPD}          {\rm{SPD}\xspace}
\newcommand{\SSD}          {\rm{SSD}\xspace}
\newcommand{\TeV}          {Te\kern-.1emV\xspace}
\newcommand{\TOF}          {\rm{TOF}\xspace}
\newcommand{\TPC}          {\rm{TPC}\xspace}
\newcommand{\TRD}          {\rm{TRD}\xspace}
\newcommand{\ttbar}{\ensuremath{{\PQt{}\overline{\PQt}}}} %Mod for ease of use
\newcommand{\twoH}         {$\sqrt{s}~=~0.2$~Te\kern-.1emV\xspace}
\newcommand{\twohundrednn}       {$\sqrt{s_{\mathrm{NN}}}~=~200$~Ge\kern-.1emV\xspace}
\newcommand{\twosevensix}  {$\sqrt{s}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\Vdecay} 	   {\ensuremath{V^{0}}\xspace}
\newcommand{\vm}[1]{\langle #1 \rangle}     % valor medio
\newcommand{\VZEROA}       {\rm{V0A}\xspace}
\newcommand{\VZEROC}       {\rm{V0C}\xspace}
\newcommand{\VZERO}        {\rm{V0}\xspace}
\newcommand{\X}            {\ensuremath{\Xi^-}\xspace}
%newcommand{\XeXe}         {\mbox{Xe--Xe}\xspace}
\newcommand{\Xis}          {\ensuremath{\Xi^{\pm}}\xspace}
\newcommand{\ycms}         {\ensuremath{y_{\rm CMS}}\xspace}
\newcommand{\y}         {\ensuremath{y}\xspace}
\newcommand{\ylab}         {\ensuremath{y_{\rm lab}}\xspace}
\newcommand{\yrange}[1]    {\mbox{$\left | y \right |~<~#1$}}
\newcommand{\ZDC}          {\rm{ZDC}\xspace}
\newcommand{\ZDCs}         {\rm{ZDCs}\xspace}
\newcommand{\ZNA}          {\rm{ZNA}\xspace}
\newcommand{\ZNC}          {\rm{ZNC}\xspace}
%\newcommand\mylessim{\ensuremath\mathrel{\raisebox{1pt}{\stackunder{$<$}{\rotatebox{-27}{\resizebox{7pt}{2pt}{$\sim$}}}}}}
\newcommand{\vn}{$v_{\mathrm{n}}$\xspace}
\newcommand{\vtwo}{\ensuremath{v_{2}}\xspace}
\newcommand{\vthree}{\ensuremath{v_{3}}\xspace}
\newcommand{\vfour}{\ensuremath{v_{4}}\xspace}
\newcommand{\vtwotwo}{\ensuremath{\vtwo\{2\}}\xspace}
\newcommand{\vtwofour}{\ensuremath{\vtwo\{4\}}\xspace}
\newcommand{\vtwosix}{\ensuremath{\vtwo\{6\}}\xspace}
\newcommand{\vtwoeight}{\ensuremath{\vtwo\{8\}}\xspace}
\newcommand{\noff}  {\ensuremath{N_\text{trk}^\text{offline}}\xspace}
\newcommand{\rootsNN} {\ensuremath{\sqrt{\smash[b]{s_{_{\mathrm{NN}}}}}}\xspace}
\newcommand{\roots} {\ensuremath{\sqrt{\smash[b]{s}}}\xspace}
\newcommand{\PbPb}{\ensuremath{\mathrm{Pb}\mathrm{Pb}}\xspace}
\newcommand{\XeXe}{\ensuremath{\mathrm{Xe}\mathrm{Xe}}\xspace}
\newcommand{\pPb}{\ensuremath{\Pp\mathrm{Pb}}\xspace}
\newcommand{\pp}{\ensuremath{\Pp\Pp}\xspace}
\newcommand{\pn}{\ensuremath{\Pp\Pn}\xspace}
\newcommand{\ppbar}{\ensuremath{\Pp\PAp}\xspace}
\newcommand{\sigmaVis}{\ensuremath{\sigma_{\text{vis}}}\xspace}
\newcommand{\mub}{\ensuremath{\,\mu\text{b}}\xspace}
\newcommand{\xthree}{\PGccDoP{3872}}
\newcommand{\stt}{\ensuremath{\sigma_{\ttbar}}\xspace}

==> Zhang_ATLAS/usepackage.tex <==
\usepackage{eucal}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage{placeins}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage[switch*]{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
 \input{usepackage.tex}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage{placeins}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage[switch*]{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[english,russian]
%\usepackage{amssymb,graphicx, subcaption}wrapfig}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{float}
\usepackage{feynmf}
\usepackage{xspace}
%\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{afterpage}
%\usepackage{hyperref}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{amsthm}
%\usepackage{color}
\usepackage{graphicx}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{lineno}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage[section]{placeins}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{xfrac}
\usepackage{transparent}
\usepackage{array}
\usepackage{placeins}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{lineno}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{float}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[utf8]{inputenc}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
%\usepackage{graphicx, subcaption}
\usepackage{graphicx}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[comma,square,numbers,sort&compress]{natbib}
\usepackage{lineno}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{subfigure}
\usepackage{hyperref}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage[utf8]{inputenc}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
%\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{float}
\usepackage{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
%\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
%\usepackage[colorinlistoftodos]{todonotes}
%\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[english,russian]
%\usepackage{amssymb,graphicx,wrapfig}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{float}
\usepackage{feynmf}	%For drawing Feynman diagrams
\usepackage{xspace}
%\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{xfrac}
\usepackage{transparent}
\usepackage{array}
\usepackage{placeins}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{afterpage}
%\usepackage{hyperref}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{amsthm}
%\usepackage{color}
\usepackage{graphicx}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{lineno}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage[section]{placeins}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{lineno}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{float}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[utf8]{inputenc}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
%\usepackage{graphicx, subcaption}
\usepackage{graphicx}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[comma,square,numbers,sort&compress]{natbib}
\usepackage{lineno}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{subfigure}
\usepackage{hyperref}
% \usepackage{caption}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage[utf8]{inputenc}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
%\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{float}
\usepackage{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
%\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
%\usepackage[colorinlistoftodos]{todonotes}
%\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
% Packages for guideline conventions
\usepackage{ptdr-definitions}
\usepackage{hepunits}
\usepackage{heppennames2}
\usepackage{lineno}

==> definecolor.tex <==
\input{definecolor.tex}
\definecolor{tab0}{HTML}{1f77b4}
\definecolor{tab1}{HTML}{ff7f0e}
\definecolor{tab2}{HTML}{2ca02c}
\definecolor{tab3}{HTML}{d62728}
\definecolor{tab4}{HTML}{9467bd}
\definecolor{tab5}{HTML}{8c564b}
\definecolor{tab6}{HTML}{e377c2}
\definecolor{tab7}{HTML}{7f7f7f}
\definecolor{tab8}{HTML}{bcbd22}
\definecolor{tab9}{HTML}{17becf}
\definecolor{c02}{HTML}{729fcf}
\definecolor{c01}{HTML}{3465a4}
\definecolor{c0}{HTML}{204a87}
\definecolor{c12}{HTML}{fcaf3e}
\definecolor{c11}{HTML}{f57900}
\definecolor{c1}{HTML}{ce5c00}
\definecolor{c22}{HTML}{8ae234}
\definecolor{c21}{HTML}{73d216}
\definecolor{c2}{HTML}{4e9a06}
\definecolor{c32}{HTML}{ef2929}
\definecolor{c31}{HTML}{cc0000}
\definecolor{c3}{HTML}{a40000}
\definecolor{c42}{HTML}{ad7fa8}
\definecolor{c41}{HTML}{75507b}
\definecolor{c4}{HTML}{5c3566}
\definecolor{c52}{HTML}{e9b96e}
\definecolor{c51}{HTML}{c17d11}
\definecolor{c5}{HTML}{8f5902}
\definecolor{c62}{HTML}{fce94f}
\definecolor{c61}{HTML}{edd400}
\definecolor{c6}{HTML}{c4a000}
\definecolor{tab0}{HTML}{1f77b4}
\definecolor{tab1}{HTML}{ff7f0e}
\definecolor{tab2}{HTML}{2ca02c}
\definecolor{tab3}{HTML}{d62728}
\definecolor{tab4}{HTML}{9467bd}
\definecolor{tab5}{HTML}{8c564b}
\definecolor{tab6}{HTML}{e377c2}
\definecolor{tab7}{HTML}{7f7f7f}
\definecolor{tab8}{HTML}{bcbd22}
\definecolor{tab9}{HTML}{17becf}
\definecolor{c02}{HTML}{729fcf}
\definecolor{c01}{HTML}{3465a4}
\definecolor{c0}{HTML}{204a87}
\definecolor{c12}{HTML}{fcaf3e}
\definecolor{c11}{HTML}{f57900}
\definecolor{c1}{HTML}{ce5c00}
\definecolor{c22}{HTML}{8ae234}
\definecolor{c21}{HTML}{73d216}
\definecolor{c2}{HTML}{4e9a06}
\definecolor{c32}{HTML}{ef2929}
\definecolor{c31}{HTML}{cc0000}
\definecolor{c3}{HTML}{a40000}
\definecolor{c42}{HTML}{ad7fa8}
\definecolor{c41}{HTML}{75507b}
\definecolor{c4}{HTML}{5c3566}
\definecolor{c52}{HTML}{e9b96e}
\definecolor{c51}{HTML}{c17d11}
\definecolor{c5}{HTML}{8f5902}
\definecolor{c62}{HTML}{fce94f}
\definecolor{c61}{HTML}{edd400}
\definecolor{c6}{HTML}{c4a000}


==> proceedings_elba2021_ragoni/commands.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% These are some new commands that may be useful 
% for paper writing in general. If other newcommands
% are needed for your specific paper, please feel 
% free to add here. 
%
% The currently available commands are organized in: 
% 1) Systems
% 2) Quantities
% 3) Energies and units
% 4) Detectors
% 5) particle species 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% 1) SYSTEMS 
\newcommand{\pp}           {pp\xspace}
\newcommand{\ppbar}        {\mbox{$\mathrm {p\overline{p}}$}\xspace}
\newcommand{\XeXe}         {\mbox{Xe--Xe}\xspace}
\newcommand{\PbPb}         {\mbox{Pb--Pb}\xspace}
\newcommand{\pA}           {\mbox{pA}\xspace}
\newcommand{\pPb}          {\mbox{p--Pb}\xspace}
\newcommand{\AuAu}         {\mbox{Au--Au}\xspace}
\newcommand{\dAu}          {\mbox{d--Au}\xspace}

% 2) QUANTITIES 
\newcommand{\s}            {\ensuremath{\sqrt{s}}\xspace}
\newcommand{\snn}          {\ensuremath{\sqrt{s_{\mathrm{NN}}}}\xspace}
\newcommand{\pt}           {\ensuremath{p_{\rm T}}\xspace}
\newcommand{\meanpt}       {$\langle p_{\mathrm{T}}\rangle$\xspace}
\newcommand{\ycms}         {\ensuremath{y_{\rm CMS}}\xspace}
\newcommand{\ylab}         {\ensuremath{y_{\rm lab}}\xspace}
\newcommand{\y}         {\ensuremath{y}\xspace}
\newcommand{\etarange}[1]  {\mbox{$\left | \eta \right |~<~#1$}}
\newcommand{\yrange}[1]    {\mbox{$\left | y \right |~<~#1$}}
\newcommand{\dndy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\dndeta}       {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}\eta}\xspace}
\newcommand{\avdndeta}     {\ensuremath{\langle\dndeta\rangle}\xspace}
\newcommand{\dNdy}         {\ensuremath{\mathrm{d}N_\mathrm{ch}/\mathrm{d}y}\xspace}
\newcommand{\Npart}        {\ensuremath{N_\mathrm{part}}\xspace}
\newcommand{\Ncoll}        {\ensuremath{N_\mathrm{coll}}\xspace}
\newcommand{\dEdx}         {\ensuremath{\textrm{d}E/\textrm{d}x}\xspace}
\newcommand{\RpPb}         {\ensuremath{R_{\rm pPb}}\xspace}

% 3) ENERGIES, UNITS
\newcommand{\nineH}        {$\sqrt{s}~=~0.9$~Te\kern-.1emV\xspace}
\newcommand{\seven}        {$\sqrt{s}~=~7$~Te\kern-.1emV\xspace}
\newcommand{\eight}        {$\sqrt{s}~=~8$~Te\kern-.1emV\xspace}
\newcommand{\twoH}         {$\sqrt{s}~=~0.2$~Te\kern-.1emV\xspace}
\newcommand{\twosevensix}  {$\sqrt{s}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\five}         {$\sqrt{s}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\fiveExactly}  {$\sqrt{s}~=~5$~Te\kern-.1emV\xspace}
\newcommand{\twosevensixnn}{$\sqrt{s_{\mathrm{NN}}}~=~2.76$~Te\kern-.1emV\xspace}
\newcommand{\fivenn}       {$\sqrt{s_{\mathrm{NN}}}~=~5.02$~Te\kern-.1emV\xspace}
\newcommand{\LT}           {L{\'e}vy-Tsallis\xspace}
\newcommand{\GeVc}         {Ge\kern-.1emV/$c$\xspace}
\newcommand{\MeVc}         {Me\kern-.1emV/$c$\xspace}
\newcommand{\TeV}          {Te\kern-.1emV\xspace}
\newcommand{\GeV}          {Ge\kern-.1emV\xspace}
\newcommand{\MeV}          {Me\kern-.1emV\xspace}
\newcommand{\GeVmass}      {Ge\kern-.05emV/$c^2$\xspace}
\newcommand{\MeVmass}      {Me\kern-.05emV/$c^2$\xspace}
\newcommand{\lumi}         {\ensuremath{\mathcal{L}}\xspace}

% 4) DETECTORS 
\newcommand{\ITS}          {\rm{ITS}\xspace}
\newcommand{\TOF}          {\rm{TOF}\xspace}
\newcommand{\ZDC}          {\rm{ZDC}\xspace}
\newcommand{\ZDCs}         {\rm{ZDCs}\xspace}
\newcommand{\ZNA}          {\rm{ZNA}\xspace}
\newcommand{\ZNC}          {\rm{ZNC}\xspace}
\newcommand{\SPD}          {\rm{SPD}\xspace}
\newcommand{\SDD}          {\rm{SDD}\xspace}
\newcommand{\SSD}          {\rm{SSD}\xspace}
\newcommand{\TPC}          {\rm{TPC}\xspace}
\newcommand{\TRD}          {\rm{TRD}\xspace}
\newcommand{\VZERO}        {\rm{V0}\xspace}
\newcommand{\VZEROA}       {\rm{V0A}\xspace}
\newcommand{\VZEROC}       {\rm{V0C}\xspace}
\newcommand{\Vdecay} 	   {\ensuremath{V^{0}}\xspace}

% 4) PARTICLE SPECIES 
\newcommand{\ee}           {\ensuremath{e^{+}e^{-}}} 
\newcommand{\pip}          {\ensuremath{\pi^{+}}\xspace}
\newcommand{\pim}          {\ensuremath{\pi^{-}}\xspace}
\newcommand{\kap}          {\ensuremath{\rm{K}^{+}}\xspace}
\newcommand{\kam}          {\ensuremath{\rm{K}^{-}}\xspace}
\newcommand{\pbar}         {\ensuremath{\rm\overline{p}}\xspace}
\newcommand{\kzero}        {\ensuremath{{\rm K}^{0}_{\rm{S}}}\xspace}
\newcommand{\lmb}          {\ensuremath{\Lambda}\xspace}
\newcommand{\almb}         {\ensuremath{\overline{\Lambda}}\xspace}
\newcommand{\Om}           {\ensuremath{\Omega^-}\xspace}
\newcommand{\Mo}           {\ensuremath{\overline{\Omega}^+}\xspace}
\newcommand{\X}            {\ensuremath{\Xi^-}\xspace}
\newcommand{\Ix}           {\ensuremath{\overline{\Xi}^+}\xspace}
\newcommand{\Xis}          {\ensuremath{\Xi^{\pm}}\xspace}
\newcommand{\Oms}          {\ensuremath{\Omega^{\pm}}\xspace}
\newcommand{\degree}       {\ensuremath{^{\rm o}}\xspace}

==> usepackage.tex <==
\usepackage{eucal}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage{placeins}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage[switch*]{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage{placeins}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage[switch*]{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[english,russian]
%\usepackage{amssymb,graphicx, subcaption}wrapfig}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{float}
\usepackage{feynmf}
\usepackage{xspace}
%\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{afterpage}
%\usepackage{hyperref}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{amsthm}
%\usepackage{color}
\usepackage{graphicx}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{lineno}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage[section]{placeins}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{xfrac}
\usepackage{transparent}
\usepackage{array}
\usepackage{placeins}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{lineno}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{float}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[utf8]{inputenc}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
%\usepackage{graphicx, subcaption}
\usepackage{graphicx}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[comma,square,numbers,sort&compress]{natbib}
\usepackage{lineno}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{subfigure}
\usepackage{hyperref}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage[utf8]{inputenc}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
%\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{float}
\usepackage{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
%\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
%\usepackage[colorinlistoftodos]{todonotes}
%\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[english,russian]
%\usepackage{amssymb,graphicx,wrapfig}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{float}
\usepackage{feynmf}	%For drawing Feynman diagrams
\usepackage{xspace}
%\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{xfrac}
\usepackage{transparent}
\usepackage{array}
\usepackage{placeins}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{afterpage}
%\usepackage{hyperref}
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{amsthm}
%\usepackage{color}
\usepackage{graphicx}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{lineno}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage[section]{placeins}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{lineno}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{float}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[utf8]{inputenc}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
%\usepackage{graphicx, subcaption}
\usepackage{graphicx}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
%\usepackage[comma,square,numbers,sort&compress]{natbib}
\usepackage{lineno}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{subfigure}
\usepackage{hyperref}
% \usepackage{caption}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage[utf8]{inputenc}
\usepackage{lineno}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
%\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{float}
\usepackage{lineno}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
%\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
%\usepackage[colorinlistoftodos]{todonotes}
%\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
\usepackage{listings}
\usepackage{xcolor}
\usepackage{multirow}
\usepackage{jheppub}  
\usepackage{dcolumn}
\usepackage[english]{babel}
\usepackage[utf8x]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{palatino}
\usepackage{amsmath}
\usepackage{afterpage}
\usepackage{graphicx, subcaption}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage[colorlinks=true]{hyperref}
\usepackage{makeidx}
% Packages for guideline conventions
\usepackage{ptdr-definitions}
\usepackage{hepunits}
\usepackage{heppennames2}
\usepackage{lineno}
